Multinucleon Short-Range Correlation Model for Nuclear Spectral Functions

The main goal of the research presented in this dissertation was to develop a theoretical model for relativistic nuclear spectral functions at high missing momenta and removal energies based on the multi-nucleon short-range correlation (SRC) model. The nuclear spectral functions are necessary for the description of high energy nuclear processes currently being studied at different labs such as JLAB, LHC and FNAL. The model followed the effective Feynman diagrammatic approach in order to account for the relativistic effects important in the SRC domain. In addition to the two-nucleon (2N) SRC with center of mass motion contribution, the contribution of the three-nucleon SRCs to the spectral functions was also derived. The latter was modeled based on the assumption that the 3N SRCs are a product of two sequential short range nucleon-nucleon (NN) interactions. The nuclear spectral functions models were derived from two theoretical frameworks for evaluating covariant Feynman diagrams: In the first, referred to as the virtual nucleon approximation, the Feynman diagrams were reduced to the time ordered non-covariant diagrams by evaluating the nucleon spectators in the SRC at their positive energy poles, neglecting explicitly the contribution from vacuum diagrams. In the second approach, referred to as the light-front approximation, the boost invariant nuclear spectral function was formulated in the light-front reference frame in which case the vacuum diagrams are kinematically suppressed and the bound nucleon is described by its light-front variables such as momentum fraction, transverse momentum and invariant mass. On the basis of the derived nuclear spectral functions, the corresponding computational models were developed from which the numerical estimates of the SRC spectral functions, the SRC momentum distributions, and the SRC density matrices were obtained.

==> 0/copyright.tex <==
\newpage
\vspace*{9cm}
\begin{center}
	\copyright \hspace{1pt} Copyright 2017 by Oswaldo Artiles\\
	All rights reserved.
\end{center}


==> 0/listFigures.tex <==
%\table of contents

\singlespacing


\hspace*{140pt} LIST OF FIGURES\\\\
FIGURE \hspace*{365pt} PAGE\\\\
\hspace*{12pt} 1.1 \hspace*{6pt} Lepton-nucleus inclusive scattering \dotfill  5\\\\
\hspace*{12pt} 1.2 \hspace*{6pt} Lepton-nucleus deep inelastic inclusive scattering regions \dotfill  8\\\\
\hspace*{12pt}  1.3 \hspace*{6pt} Theoretical predictions for the Fermi motion corrections of the bound nucleon\\
\hspace*{36pt} structure functions $F^N_2$ for iron. Figure from  \cite {Au83} \dotfill   10\\\\
\hspace*{12pt}  1.4 \hspace*{6pt} EMC experimental results for the ratio of the structure functions of iron nucleus\\
\hspace*{36pt}  and deuterium $(F^N_2(Fe)/F^N_2(D))$. Figure from  \cite {Au83} \dotfill  11\\\\
\hspace*{12pt}  1.5 \hspace*{6pt}Carbon EMC ratios for the highest $Q^2$ settings ($Q^2$ quoted at x = 0.75). Uncertain-
\hspace*{36pt}  ties are the combined statistical and point-to-point systematic. The solid curve is the\\
\hspace*{36pt}   SLAC fit to the Carbon EMC ratio. Figure from  \cite {Se09} \dotfill  12\\\\
\hspace*{12pt}  1.6 \hspace*{6pt} 2N and 3N scaling regions for nucleus A. Figure from Ref. \cite {Kim2}  \dotfill  12 \\\\
\hspace*{12pt}  1.7 \hspace*{6pt} The EMC slopes versus the SRC scale factors. Figure from Ref.
 \cite {LW1}   \dotfill  14  \\\\
\hspace*{12pt}  1.8 \hspace*{6pt} 2N and 3N SRC models for nuclear spectral functions  \dotfill  16\\\\
\hspace*{12pt}  2.1 \hspace*{6pt} Representation of the covariant Feynman amplitude through the sum of the time\\
\hspace*{36pt} ordered amplitudes. Panel (b) corresponds to the scenario in which first, the \\
\hspace*{36pt}  bound nucleon is resolved in the nucleus which interacts with the incoming probe\\
\hspace*{36pt}  $h$. In panel (c), initially, the incoming probe produces a $\bar N N$, anti-nucleon and\\
\hspace*{36pt} nucleon pair, with subsequent absorption of the $\bar N$ anti-nucleon in the nucleus. \dotfill   22\\\\
\hspace*{12pt}  2.2 \hspace*{6pt} Expansion of the nuclear spectral function into the contributions of the mean \\
\hspace*{36pt} field (a), the 2N (b) and the 3N (c) SRCs. For each case the initial nuclear tran-\\
\hspace*{36pt} sition vertices are different, corresponding to transition of $A\to N,A-1$; $A\to \\
\hspace*{36pt} NN,A-1$ and $A\to NNN,A-3$ for the mean field, the 2N and the 3N SRCs re-\\
\hspace*{36pt} spectively. The NN (b)  and NNN (c)  labels identify the 2N and the 3N SRCs with\\
 \hspace*{36pt} effective NN and NNN vertices  elaborated in the text \dotfill  27\\\\
\hspace*{12pt}  2.3 \hspace*{6pt} Diagram corresponding to the 3N SRC contribution to the nuclear  spectral func-\\
\hspace*{36pt} tions  \dotfill  29\\\\
\hspace*{12pt} 4.1 \hspace*{6pt} The momentum distribution of deuteron (s-wave: dot-dash, d-wave:dash) \dotfill   98\\\\
\hspace*{12pt} 4.2 \hspace*{6pt} Upper graph: Deuteron momentum distribution. Lower graph: Deuteron light-\\
\hspace*{36pt} front density matrix \dotfill    99\\\\
\hspace*{12pt} 4.3 \hspace*{6pt} Nuclear spectral function for $^9$Be in the nonrelativistic limit of  the VNA \dotfill  100\\\\
\hspace*{12pt} 4.4 \hspace*{6pt} Nuclear spectral function for $^{56}$Fe in the nonrelativistic limit of   the VNA  \dotfill   101\\\\
\hspace*{12pt} 4.5 \hspace*{6pt} Nuclear spectral function, with constant values of momentum for $^3$He and $^9$Be, in \\
\hspace*{36pt}   VNA and in the nonrelativistic limit of   the VNA\dotfill    102\\\\
\hspace*{12pt} 4.6 \hspace*{6pt} Nuclear spectral function for $^{9}$Be in light-front approximation, for $\tilde M^2_N = 0.5 \;\mathrm {GeV}^2$ \dotfill    103\\\\
\hspace*{12pt} 4.7 \hspace*{6pt} Nuclear spectral function for $^{197}$Au in light-front approximation, for $\tilde M^2_N = 0.2 \;\mathrm {GeV}^2$\\
\hspace*{36pt}   \dotfill    104\\\\
\hspace*{12pt} 4.8 \hspace*{6pt} SRC density matrix  for $^{9}$Be in light-front approximation \dotfill    105\\\\
\hspace*{12pt} 4.9 \hspace*{6pt} SRC density matrix  for $^{197}$Au in light-front approximation \dotfill    106\\\\
\hspace*{12pt} 4.10 \hspace*{0pt} SRC  momentum distribution  for proton in $^{3}$He, in VNA and in the nonrelativistic  \\
\hspace*{36pt}  limit of the VNA, the predictions in the nonrelativistic limit of the VNA are compa-   \\
\hspace*{36pt}  red to QMC calculations  \dotfill    110\\\\
\hspace*{12pt} 4.11 \hspace*{0pt} SRC momentum distribution for $^{8}$He in the nonrelativistic limit of the VNA compa-\\
\hspace*{36pt}  red to QMC calculations \dotfill    111\\\\
\hspace*{12pt} 4.12 \hspace*{0pt} SRC  momentum distribution  for neutron in $^{9}$Be, in VNA and in the nonrelativistic \\
\hspace*{36pt}  limit of the VNA, the predictions in the nonrelativistic limit of the VNA are compa-   \\
\hspace*{36pt} red to QMC calculations \dotfill    112\\\\
\hspace*{12pt} 4.13 \hspace*{0pt} SRC momentum distribution for $^{56}$Fe in the nonrelativistic limit of the VNA compa-\\
\hspace*{36pt} red to 2N SRC momentum distribution for proton in Ciofi/Simula [52] \dotfill    113\\\\
\hspace*{12pt} 4.14 \hspace*{0pt} SRC momentum distribution for $^{208}$Pb in VNA compared to predictions in the non-\\ 
\hspace*{36pt}  relativistic limit of the VNA \dotfill    113\\\\
\hspace*{12pt} 4.15 \hspace*{0pt} Momentum distribution for light nuclei calculated with the SRC nuclear spectral\\
 \hspace*{36pt} functions in the nonrelativistic limit of the VNA,  compared to the curve fitting ob-\\  
\hspace*{36pt}   tained with the mean field parameters in Table 4.3 and SRC parameters \;  in \; Table \\
\hspace*{36pt} 4.5 \dotfill    117\\\\
\hspace*{12pt} 4.16 \hspace*{0pt} Momentum distribution for heavy nuclei calculated with the SRC nuclear spectral\\
 \hspace*{36pt} functions  in the nonrelativistic limit of the VNA,   compared to the curve fitting ob-\\  
\hspace*{36pt}  tained with the mean field parameters in Table 4.4 and SRC parameters \;  in \; Table\\
 \hspace*{36pt} 4.6 \dotfill    118\\\\
\hspace*{12pt} 4.17 \hspace*{0pt} Momentum distribution for light nuclei calculated with the SRC nuclear spectral\\
 \hspace*{36pt} functions for VNA,  compared to the curve fitting obtained with  the mean field\\  
\hspace*{36pt}   parameters in Table 4.7 and SRC parameters  in Table 4.9 \dotfill    122\\\\
\hspace*{12pt} 4.18 \hspace*{0pt} Momentum distribution for heavy nuclei calculated with the SRC nuclear spectral\\
 \hspace*{36pt} functions for VNA,  compared to the curve fitting obtained with  the mean field\\  
\hspace*{36pt}  parameters in Table 4.8 and SRC parameters  in Table 4.10 \dotfill    123\\\\



==> 0/listTables.tex <==
%\table of contents

\singlespacing


\hspace*{140pt} LIST OF TABLES\\\\
TABLE \hspace*{370pt} PAGE\\\\
\hspace*{12pt} 4.1 \hspace*{6pt} 2N SRC parameters for light and heavy Nuclei (k$_F$ in GeV)\dotfill   107\\\\
\hspace*{12pt} 4.2 \hspace*{6pt} 3N SRC parameters for light and heavy nuclei \dotfill    108\\\\
\hspace*{12pt} 4.3 \hspace*{6pt} Parameters for the non-relativistic mean-field momentum distribution for light \\
\hspace*{36pt}   nuclei A $\le$ 12  \dotfill  115\\\\
\hspace*{12pt} 4.4 \hspace*{6pt} Parameters for the non-relativistic mean-field momentum distribution for heavy\\
\hspace*{36pt}  nuclei 16 $\le$ A $\le$ 208  \dotfill  115\\\\
\hspace*{12pt} 4.5 \hspace*{6pt} Parameters for the SRC momentum distribution in the nonrelativistic limit of the VNA\\
\hspace*{36pt}   for light nuclei A $\le$ 12  \dotfill    118\\\\
\hspace*{12pt} 4.6 \hspace*{6pt} Parameters for the SRC momentum distribution  in the nonrelativistic limit of the VNA  \\
\hspace*{36pt} for  heavy nuclei 16 $\le$ A $\le$ 208   \dotfill    118\\\\
\hspace*{12pt} 4.7 \hspace*{6pt} Parameters for  the mean-field  momentum distribution in VNA  for light nuclei A $\le$12 \\
 \hspace*{36pt}  \dotfill    119\\\\
\hspace*{12pt} 4.8 \hspace*{6pt} Parameters  for  the mean-field  momentum distribution in VNA  for heavy nuclei   \\
\hspace*{36pt} 16 $\le$ A $\le$ 208   \dotfill    119\\\\
\hspace*{12pt} 4.9 \hspace*{6pt} Parameters  for  the SRC  momentum distribution in VNA for light nuclei A $\le$12 
 \dotfill    120\\\\
\hspace*{12pt} 4.10 \hspace*{0pt} Parameters  for  the SRC  momentum distribution in VNA  for heavy nuclei  16 $\le$ A $\le$ 208\\
\hspace*{36pt}    \dotfill    120\\\\


==> 0/tableContent.tex <==
%\table of contents

\singlespacing

%{\centering {TABLE OF CONTENTS}\hfill}
%\renewcommand\contentsname{\normalfont\MakeUppercase{Table of contents}\hfill}
\hspace*{140pt} TABLE OF CONTENTS\\\\
CHAPTER \hspace*{355pt} PAGE\\\\
1 \hspace*{6pt}  Introduction \dotfill 1\\
\hspace*{12pt} 1.1 \hspace*{6pt} Lepton-nucleus inclusive scattering cross section and nuclear spectral function  \dotfill  5\\
\hspace*{12pt} 1.2 \hspace*{6pt} The Nuclear EuropeanMuon Collaboration (EMC) Effect  \dotfill  9\\
\hspace*{12pt}  1.3 \hspace*{6pt} Multinucleon short-range correlations in nuclei  \dotfill   11\\
\hspace*{12pt}  1.4 \hspace*{6pt} Nuclear spectral function model \dotfill  18\\\\
 2 \hspace*{6pt} Multinucleon short-range correlation model for nuclear spectral functions: Theoretical\\
\hspace*{14pt} framework \dotfill   20\\
\hspace*{12pt}  2.1 \hspace*{6pt} Approaches to deal with vacuum fluctuations  \dotfill   21\\
\hspace*{12pt}  2.2 \hspace*{6pt} Diagrammatic approach for modeling nuclear spectral functions \dotfill  26\\
\hspace*{12pt}  2.3 \hspace*{6pt} Nuclear spectral function in virtual nucleon approximation  \dotfill  31\\
\hspace*{12pt}  2.4 \hspace*{6pt} Nuclear spectral function in light-front approximation  \dotfill 45\\
\hspace*{12pt}  2.5 \hspace*{6pt} Summary \dotfill 68\\\\
3 \hspace*{6pt} Multinucleon short-range correlation model for nuclear spectral functions: Models
for\\
\hspace*{14pt} numerical computation \dotfill   70\\
\hspace*{12pt} 3.1 \hspace*{6pt} Computational models for SRC nuclear spectral function in virtual nucleon\\
\hspace*{36pt} approximation \dotfill    71\\
\hspace*{12pt} 3.2 \hspace*{6pt} Computational models for SRC nuclear spectral function in light-front\\
\hspace*{36pt} approximation \dotfill    77\\
\hspace*{12pt} 3.3 \hspace*{6pt} Computational models for SRC nuclear spectral function in nonrelativistic\\
\hspace*{36pt} approximation \dotfill    86\\
\hspace*{12pt} 3.4 \hspace*{6pt} Summary \dotfill    92\\\\
4 \hspace*{6pt} Numerical estimates of nuclear spectral functions, density matrices and momentum\\
\hspace*{14pt} distributions \dotfill   94\\
\hspace*{12pt} 4.1 \hspace*{6pt} Parameters for numerical estimates of the nuclear spectral functions \dotfill   95\\
\hspace*{12pt} 4.2 \hspace*{6pt} Momentum distribution and light-front density matrix for deuteron \dotfill    97\\
\hspace*{12pt} 4.3 \hspace*{6pt} Numerical estimates for SRC nuclear spectral function in virtual nucleon\\
\hspace*{36pt} approximation \dotfill    99\\
\hspace*{12pt} 4.4 \hspace*{6pt} Numerical estimates for SRC nuclear spectral function in light-front\\
\hspace*{36pt} approximation \dotfill   102\\
\hspace*{12pt} 4.5 \hspace*{6pt} Numerical estimates for SRC density matrices in light-front approximation \dotfill    105\\
\hspace*{12pt} 4.6 \hspace*{6pt} Numerical estimates for SRC momentum distribution in virtual nucleon\\
\hspace*{36pt} approximation \dotfill    107\\
\hspace*{12pt} 4.7 \hspace*{6pt} Parametrization of SRC and mean field momentum distribution \dotfill    114\\
\hspace*{12pt} 4.8 \hspace*{6pt} Summary \dotfill   123\\\\
5 \hspace*{6pt} Conclusions \dotfill    125\\
\hspace*{12pt} 5.1 \hspace*{6pt} Application of the multi-nucleon short range correlation model for the nuclear\\
\hspace*{36pt} spectral functions \dotfill  128\\\\
Bibliography \dotfill   130\\\\
VITA \dotfill   138\\


==> 1/NuTeV.tex <==
The  neutral  gauge fields $B_\mu$ and $W^3_\mu$  of the electro-weak standard model are related to the electromagnetic field $A_\mu$ and the neutral weak boson  field  $Z_\mu$ by 
\begin{align}
\tiny
 A_\mu  &= B_\mu \cos \theta_W + W^3_\mu \sin \theta_W\nonumber\\
 Z_\mu &= -B_\mu \sin \theta_W + W^3_\mu \cos \theta_W
\normalsize
\end{align}
where  $ \theta_W$ is the weak angle \cite {PDG12b}.  The experimental value of  this angle for free nucleons is  $\sin^2 \theta_W = $ 0.2227 $\pm$ 0.0004 \cite {CERN02}. The NuTeV collaboration  found an experimental  value of $\sin^2 \theta_W = $ 0.2277 $\pm$ 0.0013 (stat) $\pm$ 0.0009 (syst) for bound nucleons if $^{56}$Fe nucleus, approximately three standard deviations  above  the  value for a free nucleon. This result is known as the NuTeV anomaly \cite {GPZ02}.   We will give an explanation to these results based on the presence of more energetics protons in neutron rich, large A,  asymmetric nuclei which implies that u-quarks are more modified than d-quarks, resulting in  a negative correction for the experimental value of  $\sin^2 \theta_W $ for bound nucleons.





==> 1/Relativistic.tex <==
 \section {Relativistic effects}
 \label {sec:Relativ}
 











  
  


==> 1/introductionProposal.tex <==

%\textcolor{bokunoaka}{(Should have a few orienting paragraphs)}

%\section{Quantum chromodynamics}

\pagenumbering{arabic}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Orienting paragraphs

The scattering of electrons off  nucleons and nuclei have been the most important experimental tool to study the nuclear   structure.  In 1968, the first results from deep inelastic scattering experiments  demonstrate that protons and neutrons are composite structures  made up of particles  with fractional electric charge as well as neutral particles \cite  {Fr97, Bj97}. The charged particles were later identified with the quarks predicted by Gell-Mann \cite {GE64} and Zweig \cite {ZW64a, ZW64b}, and the neutral particles with the massless gluons, the carrier of the strong interaction between quarks in hadrons.  All these experimental and theoretical efforts resulted  in the formalization and acceptance of  the theory of strong interactions: quantum chromodynamics (QCD), on which the physical hadrons are many-body, highly relativistic systems composed of light quarks and massless gluons  \cite {BRDH91, isosrc}. The proposed research is focused in the investigation of quantum chromodynamics in the nuclear medium with the main emphasis on nucleon-nucleon interaction at short distances. This type of  interaction  prevents two nucleons from coming very close together demanding the existence of high momentum components in the nuclear ground state wave function. These cannot be described in the context of nuclear mean field models and are commonly called multi-nucleon short-range correlations (SRC) \cite {AHR12}.  

Deep inelastic scattering (DIS) of leptons off  the nucleus provides information about the quark distributions in nuclei through the measurements of cross sections.   The fact that the quark momentum distributions for individual nucleons are modified in the nuclear medium was first observed by the European Muon Collaboration (EMC) experiment and is usually known as the EMC effect  \cite {Au83}. The first part of our research is  focused on understanding the role of the SRCs in the EMC effects. To incorporate the nuclear and quantum chromodynamics  efects we need  to develop a   covariant relativistic model  of nuclear  spectral function  that describes the momentum distributions and  energies of nucleons (protons and neutrons) in nuclei relevant to the whole momentum  range,  including the multi-nucleon short-range correlations (SRCs). This model is then used  in   the  derivation of the formalisms for lepton-nucleon and lepton-nucleus   elastic and inelastic scattering, needed for the calculation of the corresponding cross sections.  The   models and formalisms will be used to  provide explanations  of two important problems, the first  in  nuclear quantum chromodynamics (QCD),   and  the second  in electroweak physics.  Our first goal is  to provide  theoretical explanations   of the causes of   the strong correlation between the modification of quarks  momentum distribution of nucleons in the nucleus (nuclear EMC effect) and the nucleon-nucleon short range correlation (2N SRC)  specially for heavy  asymmetric nuclei.  This part of our research will  be a  contribution to the understanding of the nuclear quantum chromodynamics (QCD) structure at short distances in nuclei  \cite {MS0912}. The second problem to be addressed is  the discrepancy found between measurements of $\sin^2 \theta_w$ ($ \theta_w$ is the weak  angle)  involving free particles and those made for bound particles in the nuclear medium, the so-called  NuTev anomaly \cite {GPZ02}. 






==> 4/3HeSpec.tex <==

\section{Comparison\; with\; \textit {ab initio}\; $^3$He\; spectral\; function } 
\label{sec:3HeSpec}
Calculations of high momentum nuclear spectral function for constant missing momentum for $^{3}$He, obtained with our model and with an \textit {ab initio} wave  function for   $^{3}$He are included in this section. 


==> 4/ParDmLFA.tex <==

\section{Parametrization\; of\;  SRC\; density\; matrices\;in\; light-front\; approximation} 
\label{sec:ParDmLFA}



==> 4/ParSpec.tex <==

\section{Parametrization\; of\;  SRC\; nuclear\; spectral\; function } 
\label{sec:ParSpec}



==> 4/ParSpecLFA.tex <==

\subsection{Parametrization\; of\;  SRC\; nuclear\; spectral\; function\;in\; light-front\\ approximation} 
\label{sec:ParSpecLFA}



==> 4/ParSpecNRA.tex <==

\subsection{Parametrization\; of\;  SRC\; nuclear\; spectral\; function\;in\; nonrelativistic\; approximation} 
\label{sec:ParSpecNRA}



==> 4/ParSpecVNA.tex <==

\subsection{Parametrization\; of\;  SRC\; nuclear\; spectral\; function\;in\; virtual\; nucleon\\ approximation} 
\label{sec:ParSpecVNA}


